New constraints on the minimum mass for thermonuclear lithium burning in brown dwarfs

The theory of substellar evolution predicts that there is a sharp mass boundary between lithium and non-lithium brown dwarfs, not far below the substellar-mass limit. The imprint of thermonuclear burning is carved on the surface lithium abundance of substellar-mass objects during the first few hundred million years of their evolution, leading to a sharp boundary between lithium and non-lithium brown dwarfs, so-called, the lithium test. New optical spectroscopic observations of the binaries DENIS+J063001.4-184014 and DENIS+J225210.7-173013 obtained using the 10.4-m Gran Telescopio de Canarias are reported here. They allow us to re-determine their combined optical spectral types (M9.5 and L6.5, respectively) and to search for the presence of the LiI resonance doublet. The non detection of the LiI feature in the combined spectrum of DENIS\,J063001.4$-$184014AB is converted into estimates for the depletion of lithium in the individual components of this binary system. In DENIS\,J225210.7$-$173013AB we report the detection of a weak LiI feature which we tentatively ascribe as arising from the contribution of the T3.5-type secondary. Combining our results with data for seven other brown dwarf binaries in the literature treated in a self-consistent way, we confirm that there is indeed a sharp transition in mass for lithium depletion in brown dwarfs, as expected from theoretical calculations. We estimate such mass boundary is observationally located at 51.48$^{+0.22}_{-4.00}$ $M_\mathrm{Jup}$, which is lower than the theoretical determinations.

==> 00README.XXX.tex <==
nohypertex
